Complex organic molecules detected in twelve high-mass star-forming regions with Atacama Large Millimeter/submillimeter Array (ALMA)

Recent astrochemical models and experiments have explained that complex organic molecules (COMs; molecules composed of six or more atoms) are produced on the dust grain mantles in cold and dense gas in prestellar cores. However, the detailed chemical processes and the roles of physical conditions on chemistry are still far from understood. To address these questions, we investigated twelve high-mass star-forming regions using the ALMA band 6 observations. They are associated with 44/95GHz class I and 6.7 GHz class II CH$_{3}$OH masers, indicative of undergoing active accretion. We found 28 hot cores with COMs emission among 68 continuum peaks at 1.3 mm and specified 10 hot cores associated with 6.7 GHz class II CH$_{3}$OH masers. Up to 19 COMs are identified including oxygen- and nitrogen-bearing molecules and their isotopologues in cores. The derived abundances show a good agreement with those from other low- and high-mass star-forming regions, implying that the COMs chemistry is predominantly set by the ice chemistry in the prestellar core stage. One clear trend is that the COMs detection rate steeply grows with the gas column density, which can be attributed to the efficient formation of COMs in dense cores. In addition, cores associated with a 6.7 GHz class II CH$_{3}$OH maser tend to be enriched with COMs. Finally, our results suggest that the enhanced abundances of several molecules in our hot cores could be originated by the active accretion as well as different physical conditions of cores.

==> s3_f4_rotation_diagram_all_not_complied.tex <==

% - - - - rotation diagram - - - - % 
% BEFORE USING THEM, ONE HAS TO CHECK THE BAD FITTING 
% SUGGESTED CRITERIA
% Eu RANGE > 50 K 
% FITTING ERROR SMALLER THAN 0.3*VALUE (LESS THAN 3 SIGMA)
% REMOVE N_tot VALUES IN THE FIGURE

\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G10.32-0.26_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G10.32-0.26_4_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G10.34-0.14_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G10.34-0.14_2_CH3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G10.34-0.14_3_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G18.34+1.78_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G18.34+1.78_2_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G18.34+1.78_3_CH3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G18.34+1.78_8_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G18.34+1.78SW_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G18.34+1.78SW_2_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G23.43-0.18_1_CH3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G23.43-0.18_2_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G24.33+0.14_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G25.82-0.17_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G27.36-0.16_1_CH3OH.png}\\
\caption{Rotation diagram for CH$_{3}$OH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}


 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G28.37+0.07_2_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G28.37+0.07_3_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G28.37+0.07_5_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G28.37+0.07_6_CH3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G29.91-0.03_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G29.91-0.03_2_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G30.70-0.07_1_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_1_CH3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_2_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_3_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_4_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_6_CH3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_7_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_8_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_12_CH3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OH/G49.49-0.39_13_CH3OH.png}\\
\caption{Rotation diagram for CH$_{3}$OH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}


 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G10.34-0.14_1_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G10.34-0.14_2_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G10.34-0.14_3_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G18.34+1.78SW_2_C13H3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G23.43-0.18_1_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G23.43-0.18_2_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G24.33+0.14_1_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G25.82-0.17_1_C13H3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G27.36-0.16_1_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G28.37+0.07_2_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G49.49-0.39_1_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G49.49-0.39_2_C13H3OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G49.49-0.39_3_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G49.49-0.39_4_C13H3OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3OH/G49.49-0.39_6_C13H3OH.png}
\caption{Rotation diagram for $^{13}$CH$_{3}$OH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}


 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G10.34-0.14_1_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G10.34-0.14_2_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G10.34-0.14_3_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G18.34+1.78SW_2_CH318OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G23.43-0.18_1_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G23.43-0.18_2_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G24.33+0.14_1_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G25.82-0.17_1_CH318OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G27.36-0.16_1_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G28.37+0.07_2_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G49.49-0.39_1_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G49.49-0.39_2_CH318OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G49.49-0.39_3_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G49.49-0.39_4_CH318OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH318OH/G49.49-0.39_6_CH318OH.png}
\caption{Rotation diagram for CH$_{3}^{18}$OH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G10.34-0.14_1_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G10.34-0.14_2_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G10.34-0.14_3_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G18.34+1.78SW_1_CH2DOH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G18.34+1.78SW_2_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G18.34+1.78_8_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G23.43-0.18_1_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G23.43-0.18_2_CH2DOH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G24.33+0.14_1_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G25.82-0.17_1_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G27.36-0.16_1_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G28.37+0.07_2_CH2DOH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G49.49-0.39_1_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G49.49-0.39_2_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G49.49-0.39_3_CH2DOH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH2DOH/G49.49-0.39_4_CH2DOH.png}
\caption{Rotation diagram for CH$_{2}$DOH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G10.34-0.14_1_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G10.34-0.14_2_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G10.34-0.14_3_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G18.34+1.78SW_2_CH3CHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G18.34+1.78_8_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G23.43-0.18_1_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G23.43-0.18_2_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G24.33+0.14_1_CH3CHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G25.82-0.17_1_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G27.36-0.16_1_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G28.37+0.07_2_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G49.49-0.39_1_CH3CHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G49.49-0.39_2_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G49.49-0.39_3_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G49.49-0.39_4_CH3CHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3CHO/G49.49-0.39_6_CH3CHO.png}
\caption{Rotation diagram for CH$_{3}$CHO}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G10.32-0.26_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G10.32-0.26_4_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G10.34-0.14_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G10.34-0.14_2_CH3OCHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G10.34-0.14_3_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G18.34+1.78SW_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G18.34+1.78SW_2_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G18.34+1.78_1_CH3OCHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G18.34+1.78_2_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G18.34+1.78_8_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G23.43-0.18_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G23.43-0.18_2_CH3OCHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G24.33+0.14_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G25.82-0.17_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G27.36-0.16_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G28.37+0.07_2_CH3OCHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G28.37+0.07_3_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G28.37+0.07_6_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G29.91-0.03_2_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G30.70-0.07_1_CH3OCHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G49.49-0.39_1_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G49.49-0.39_2_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G49.49-0.39_3_CH3OCHO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G49.49-0.39_4_CH3OCHO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCHO/G49.49-0.39_6_CH3OCHO.png}
\caption{Rotation diagram for CH$_{3}$OCHO}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}


 
\begin{figure*}
\centering
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G10.32-0.26_1_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G10.32-0.26_4_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G10.34-0.14_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G10.34-0.14_2_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G10.34-0.14_3_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G18.34+1.78SW_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G18.34+1.78SW_2_CH3OCH3.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G18.34+1.78_1_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G18.34+1.78_2_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G18.34+1.78_3_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G18.34+1.78_8_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G23.43-0.18_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G23.43-0.18_2_CH3OCH3.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G24.33+0.14_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G25.82-0.17_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G27.36-0.16_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G28.37+0.07_2_CH3OCH3.png}\\
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G28.37+0.07_3_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G28.37+0.07_5_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G28.37+0.07_6_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G29.91-0.03_2_CH3OCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G30.70-0.07_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G49.49-0.39_1_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G49.49-0.39_2_CH3OCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G49.49-0.39_3_CH3OCH3.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3OCH3/G49.49-0.39_4_CH3OCH3.png}
\caption{Rotation diagram for CH$_{3}$OCH$_{3}$}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

 
\begin{figure*}
\centering
% \includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G10.34-0.14_1_CH3COCH3.png}
% \includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G18.34+1.78SW_2_CH3COCH3.png}
% \includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G23.43-0.18_1_CH3COCH3.png}
% \includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G23.43-0.18_2_CH3COCH3.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G24.33+0.14_1_CH3COCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G25.82-0.17_1_CH3COCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G27.36-0.16_1_CH3COCH3.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G28.37+0.07_2_CH3COCH3.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G49.49-0.39_1_CH3COCH3.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G49.49-0.39_2_CH3COCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G49.49-0.39_3_CH3COCH3.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/CH3COCH3/G49.49-0.39_4_CH3COCH3.png}
\caption{Rotation diagram for CH$_{3}$COCH$_{3}$}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}


 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G10.34-0.14_1_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G10.34-0.14_2_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G10.34-0.14_3_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G18.34+1.78SW_2_C2H5OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G18.34+1.78_8_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G23.43-0.18_1_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G23.43-0.18_2_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G24.33+0.14_1_C2H5OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G25.82-0.17_1_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G27.36-0.16_1_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G28.37+0.07_2_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G49.49-0.39_1_C2H5OH.png} \\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G49.49-0.39_2_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G49.49-0.39_3_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G49.49-0.39_4_C2H5OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C2H5OH/G49.49-0.39_6_C2H5OH.png}
\caption{Rotation diagram for C$_{2}$H$_{5}$OH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G10.34-0.14_1_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G10.34-0.14_3_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G18.34+1.78SW_2_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G23.43-0.18_1_aGg_CH2OH_2.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G23.43-0.18_2_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G24.33+0.14_1_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G25.82-0.17_1_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G27.36-0.16_1_aGg_CH2OH_2.png}\\
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G28.37+0.07_2_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G49.49-0.39_1_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G49.49-0.39_3_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G49.49-0.39_4_aGg_CH2OH_2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/aGg_CH2OH_2/G49.49-0.39_6_aGg_CH2OH_2.png}
\caption{Rotation diagram for aGg$'$-(CH$_{2}$OH)$_{2}$}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}


 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G18.34+1.78SW_2_HCOCH2OH.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G23.43-0.18_1_HCOCH2OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G23.43-0.18_2_HCOCH2OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G24.33+0.14_1_HCOCH2OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G25.82-0.17_1_HCOCH2OH.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G27.36-0.16_1_HCOCH2OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G49.49-0.39_1_HCOCH2OH.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G49.49-0.39_2_HCOCH2OH.png}\\
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G49.49-0.39_3_HCOCH2OH.png}
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G49.49-0.39_4_HCOCH2OH.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/HCOCH2OH/G49.49-0.39_6_HCOCH2OH.png}
\caption{Rotation diagram for HCOCH$_{2}$OH}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

 
\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G10.34-0.14_1_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G10.34-0.14_2_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G10.34-0.14_3_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G18.34+1.78SW_2_C13H3CN.png}\\
%\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G18.34+1.78_8_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G23.43-0.18_1_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G23.43-0.18_2_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G24.33+0.14_1_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G25.82-0.17_1_C13H3CN.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G27.36-0.16_1_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G28.37+0.07_2_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G49.49-0.39_1_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G49.49-0.39_2_C13H3CN.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G49.49-0.39_3_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G49.49-0.39_4_C13H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/C13H3CN/G49.49-0.39_6_C13H3CN.png}
\caption{Rotation diagram for $^{13}$CH$_{3}$CN}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G18.34+1.78SW_2_CH3NCO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G24.33+0.14_1_CH3NCO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G25.82-0.17_1_CH3NCO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G27.36-0.16_1_CH3NCO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_1_CH3NCO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_2_CH3NCO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_3_CH3NCO.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_4_CH3NCO.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_6_CH3NCO.png}
\caption{Rotation diagram for CH$_{3}$NCO.}
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G24.33+0.14_1_CH3NH2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G25.82-0.17_1_CH3NH2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G27.36-0.16_1_CH3NH2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_1_CH3NH2.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_2_CH3NH2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_3_CH3NH2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_4_CH3NH2.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_6_CH3NH2.png}
\caption{Rotation diagram for CH$_{2}$NH$_{3}$. }
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G10.34-0.14_1_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G10.34-0.14_2_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G23.43-0.18_1_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G23.43-0.18_2_C2H3CN.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G24.33+0.14_1_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G25.82-0.17_1_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G27.36-0.16_1_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_1_C2H3CN.png}\\
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_2_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_3_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_4_C2H3CN.png}
\includegraphics[clip,width=0.23\textwidth,keepaspectratio]{rotation_diagram/NCOMs/G49.49-0.39_6_C2H3CN.png}
\caption{Rotation diagram for C$_{2}$H$_{3}$CN. }
%\textcolor{red}{(The figure will be updated with beam filling factor of 1 and intensity unit in y scale)}
%\label{}
\end{figure*}

==> s3_tab4_rotation_diagram.tex <==

\startlongtable
\begin{deluxetable*}{lcc} 
\tablecaption{Rotation Diagram Analysis\label{tab:rot_diagram_ch3oh}}
\tabletypesize{\scriptsize}
\tablehead{									
\colhead{ } &	\multicolumn{2}{c}{CH$_{3}$OH} \\
\colhead{ } &	\colhead{T$_{\rm rot}$[K]} 	&	\colhead{N[$\rm cm^{-2}$]} }
\startdata
G10.32-0.26 C1   &    147.2$\pm$28.9 &  1.15$\pm$0.39E+17   \\ 
G10.32-0.26 C4   &    109.8$\pm$15.1 &  1.19$\pm$0.24E+17   \\ 
G10.34-0.14 C1   &    235.1$\pm$25.5 &  9.13$\pm$0.51E+17 \\ 
G10.34-0.14 C2   &    202.3$\pm$6.7 &  6.46$\pm$0.21E+17  \\ 
G10.34-0.14 C3   &    158.6$\pm$5.3 &  1.30$\pm$0.06E+18  \\ 
G18.34+1.78 C1   &    179.9$\pm$15.0 &  9.19$\pm$0.98E+16  \\ 
G18.34+1.78 C2   &    128.7$\pm$7.1 &  2.67$\pm$0.10E+17 \\ 
G18.34+1.78 C3   &    138.5$\pm$36.9 &  5.75$\pm$3.42E+16   \\ 
G18.34+1.78 C8   &    226.7$\pm$12.5 &  2.92$\pm$0.19E+17   \\ 
G18.34+1.78SW C1   &    173.6$\pm$10.9 &  1.15$\pm$0.10E+17   \\ 
G18.34+1.78SW C2   &    235.5$\pm$9.0 &  9.66$\pm$0.35E+17  \\ 
G23.43-0.18 C1   &    182.5$\pm$5.9 &  1.55$\pm$0.06E+18  \\ 
G23.43-0.18 C2   &    184.9$\pm$2.5 &  1.29$\pm$0.02E+18 \\ 
G24.33+0.14 C1   &    254.5$\pm$6.4 &  4.96$\pm$0.11E+18  \\ 
G25.82-0.17 C1   &    225.3$\pm$3.6 &  3.57$\pm$0.05E+18 \\
G27.36-0.16 C1   &    261.4$\pm$3.7 &  5.15$\pm$0.08E+18  \\
G28.37+0.07 C2   &    174.8$\pm$3.1 &  1.71$\pm$0.04E+18 \\ 
G28.37+0.07 C3   &    186.3$\pm$27.3 &  1.07$\pm$0.21E+17 \\ 
G28.37+0.07 C5   &    127.0$\pm$29.8 &  5.33$\pm$2.16E+16  \\ 
G28.37+0.07 C6   &    171.3$\pm$14.9 &  2.02$\pm$0.24E+17  \\ 
G29.91-0.03 C1   &    132.9$\pm$32.3 &  3.63$\pm$1.74E+16 \\ 
G29.91-0.03 C2   &    171.9$\pm$14.2 &  7.45$\pm$0.89E+16   \\ 
G30.70-0.07 C1   &    169.9$\pm$31.7 &  1.13$\pm$0.26E+17 \\ 
G49.49-0.39 C1   &    225.8$\pm$4.2 &  8.20$\pm$0.14E+18  \\
G49.49-0.39 C2   &    180.9$\pm$8.4 &  5.38$\pm$0.31E+18  \\ 
G49.49-0.39 C3   &    193.8$\pm$3.8 &  2.53$\pm$0.06E+18 \\
G49.49-0.39 C4   &    211.3$\pm$3.5 &  2.25$\pm$0.04E+18  \\ 
G49.49-0.39 C6   &    203.9$\pm$6.2 & 10.16$\pm$0.33E+18  \\ 
G49.49-0.39 C7  &    149.3$\pm$9.0 &  6.98$\pm$0.70E+17  \\ 
G49.49-0.39 C8   &    131.8$\pm$13.5 &  1.99$\pm$0.27E+17  \\ 
G49.49-0.39 C12  &    207.5$\pm$16.9 &  7.07$\pm$0.60E+17  \\ 
G49.49-0.39 C13   &    176.9$\pm$17.4 &  3.80$\pm$0.43E+17 
\enddata
\end{deluxetable*}

